The SAME score: Improved cosine based bias score for word embeddings

With the enourmous popularity of large language models, many researchers have raised ethical concerns regarding social biases incorporated in such models. Several methods to measure social bias have been introduced, but apparently these methods do not necessarily agree regarding the presence or severity of bias. Furthermore, some works have shown theoretical issues or severe limitations with certain bias measures. For that reason, we introduce SAME, a novel bias score for semantic bias in embeddings. We conduct a thorough theoretical analysis as well as experiments to show its benefits compared to similar bias scores from the literature. We further highlight a substantial relation of semantic bias measured by SAME with downstream bias, a connection that has recently been argued to be negligible. Instead, we show that SAME is capable of measuring semantic bias and identify potential causes for social bias in downstream tasks.

==> requirements.tex <==
\label{sec:requirements}

\subsection{Motivation}
\label{sec:req_motivation}
To emphasize the need of requirements for bias scores, we start with an example where \weat\ behaves counter-intuitive: Consider the example of gender bias with $A$ containing embeddings of male terms and $B$ containing those of female terms, and 6 occupations, half of those stereotypically male/female. All words were embedded with BERT\footnote{'bert-base-uncased' from https://huggingface.co/models}. We compute \weatw\ of the 6 occupations. The results are shown in Figure \ref{fig:weat_pretest}. 

\begin{figure}[ht]
	\centering
	\includegraphics[scale=0.25]{figures/weat_pretest}
	\caption{Bias of stereotypical male and female jobs as indicated by \weatw, which was calculated on BERT embeddings. Differences along the y-axis are an arbitrary shift for better visibility. The lower the \weatw\ score, the more female associated, the higher the \weatw\ score, the more male associated is a word.}
	\label{fig:weat_pretest}
\end{figure}

We further use groups $X = \{\mathbf{footballer},\mathbf{bishop}\}$ and $Y = \{\mathbf{hairdresser}, \mathbf{sociologist}\}$, i.e. the moderately biased occupations, as target words and measure \weat$(X,Y) = 1.7299$, which indicates a high stereotype regarding the groups $X$ and $Y$.\\
Furthermore, we construct groups $X' = \{\mathbf{footballer},\mathbf{lawmaker}\}$ and $Y' = \{\mathbf{hairdresser}, \mathbf{nurse}\}$, replacing one of the moderately biased occupations with the one that is more extremely biased according to \weatw. Now, when computing \weat\ using $X'$ and $Y'$ instead of their counterparts, one would expect a bias score to report an even larger bias with respect to these groups.\\
However, we find \weat$(X',Y') = 1.5962$. This shows that \weat's results cannot reliably be interpreted as a quantitative measure for bias.

\subsection{Overview of Requirements}

In this work, we introduce two fundamental requirements that bias scores should fulfill in order to produce meaningful measurements of bias. One is \emph{comparability} between different embeddings, the other \emph{trustworthiness} to report any present biases. Both are necessary for reliable bias quantification and reveal deficits in bias scores from the literature.

In Table \ref{tab:overview}, we provide an overview over the cosine based scores from the literature as well as our proposed score to highlight which requirements they meet. SAME is the only score to fulfill both requirements consistently.

In the following sections, we explain both criteria and their relevance for bias scores. Then we point out how the bias scores from the literature satisfy or miss these requirements.\\
Both requirements apply the following intuition of bias (based on Section \ref{sec:bias_definition} and very similar to WEAT): We observe bias of neutral words or a set of neutral words w.r.t. an arbitrary number of groups, each represented by a set of attributes. The association of a word $\mathbf{w}$ with a group is given by the mean cosine similarity with the groups attributes $mean_{\mathbf{a_i} \in A_i} cos(\mathbf{w},\mathbf{a_i})$ with $A_i$ the set of attributes describing group $i$. We consider $\mathbf{w}$ biased if it has different associations with two or more groups. On the other hand, $\mathbf{w}$ is unbiased w.r.t a set of groups if and only if it has an equal association with each one of these groups, i.e. it is equidistant to all groups.\\

\begin{table}[t] 
\centering
\caption{Overview over the properties of bias scores.}
\label{tab:overview}
\begin{tabular}{ ccc ccc }
\toprule
bias score & comparable & trustworthy & bias score & comparable & trustworthy \\
\cmidrule(r){1-3} \cmidrule(l){4-6}
\weatw &  x & \checkmark & \weat &  \checkmark & x  \\
%\hline
\macw & x & x & \mac &  x & x \\
%\hline
\dbw & \checkmark & x & \db &  \checkmark & x \\
%\hline
\samew & \checkmark & \checkmark & \same & \checkmark & \checkmark \\
\bottomrule
\end{tabular}
\end{table}


\subsection{Comparable bias scores}
\label{sec:comparable}
We introduce the novel property of \emph{comparability} of bias scores for different embedding spaces. This is relevant when evaluating biases in different embedding models (like May et al. \cite{seat}) or when evaluating debiasing methods, which change the relevant embeddings (like Liang et al.  \cite{sentdebias}). A proper bias score needs to be sensitive towards the relation of neutral words towards a bias direction (obtained by selected attributes), while being invariant to other embedding properties like the relations of attributes towards each other, embedding dimensions or average vector lengths in the embedding space.

\textbf{\weatw\ is not comparable:} 
In this regard, \weatw\ has a severe flaw as its range depends on the relation of attribute groups towards each other in the embedding space. This is illustrated by Figure \ref{fig:bias_example_angles}. Computing  \weatw$(\mathbf{secretary})$ with $A = \{\mathbf{she}\}$ and $B = \{\mathbf{he}\}$, we can insert the angles from the figure to transform  \weatw\ into:
\begin{align}
    |s(\mathbf{w},A,B)| &=& |cos(\alpha) - cos(\theta - \alpha)|
\end{align}
In fact, this functions extreme values depend on $\theta$. The smaller $\theta$, the smaller the range in which biases can be reported with this score. This means if an embedding space $E_1$ represents bias attribute groups (in the example the words "he" and "she") closer to each other than embedding space $E_2$, then  \weatw\ will report lower biases for embedding space $E_1$ in general. Hence we cannot compare biases between different embedding spaces using \weatw.\\
Using \weat\ to report biases over sets of words, solves the problem of \weatw\ by normalizing over the standard deviation. One can substantiate this with a formal proof, but this is subject to other works.

\textbf{$\mathbf{MAC}_{word}$ and $\mathbf{MAC}$ are not comparable:}
Similar to \weatw\ the MAC score depends on the relation of attributes. Considering the example from Figure \ref{fig:bias_example_angles}, MAC would report \macw$(\mathbf{secretary}) = 1 - \frac{1}{2} (cos(\alpha) + cos(\theta - \alpha))$, which clearly depends on $\theta$. Hence we cannot compare biases between different embedding spaces using \macw. The same applies to \mac\ since computing the mean over word biases does not solve this problem.

\textbf{$\mathbf{Direct Bias}_{word}$ and $\mathbf{Direct Bias}$ are comparable:}
\db\ and \dbw\ on the other hand are normalized to the interval $[0,1]$ by computing the (mean) cosine of words and the bias direction. Hence, the bias score can reach both of its extreme values solely based on the correlation of words with the bias direction but independent of the distance between attributes.

\begin{figure}[t]
\centering
   \begin{subfigure}{.32\textwidth}
    \centering
	\includegraphics[scale=0.15]{figures/bias_example_angles}
	\caption{Simplified visualization of gender stereotypes in embeddings. The occupation vectors are biased towards the respective gender if $0 < \alpha < \frac{\theta}{2}$ or $0 < \beta < \frac{\theta}{2}$.}
	\label{fig:bias_example_angles}
   \end{subfigure}
   \begin{subfigure}{.32\textwidth}
    \centering
	\includegraphics[scale=0.15]{figures/bias_example_direction}
     \caption{Example where individual bias direction differ extremely, leading to different results for the bias direction by PCA and mean.}
     \label{fig:bias_example_direction}
   \end{subfigure}
   \begin{subfigure}{.32\textwidth}
    \centering
	\includegraphics[scale=0.15]{figures/bias_example_weat}
     \caption{Example of gender-biased occupations, where WEAT's effect size fails to report bias.}
     \label{fig:bias_example_weat}
   \end{subfigure}%
\caption{Examples where the cosine based scores from the literature do not meet the requirements of comparability or trustworthiness.}
\label{fig:bias_examples}
\end{figure}



\subsection{Trustworthy bias scores}
\label{sec:trustworthy}
The second novel property of bias scores introduced in this paper is being \emph{trustworthy} to report any biases present in the embeddings and to report no bias if none is present. A trustworthy bias score must always report a bias if there is at least one biased word in the set (i.e. the word is not equidistant to all attribute sets). On the other hand if all words are unbiased (equidistant to all attribute sets), then the bias score must report no bias.

\textbf{\weat\ is not trustworthy:} 
\weatw\ is trustworthy to report such biases, as it is defined accordingly to the definition by contrasting over two attribute sets. However, \weat\ is not.
One example, where it fails to report bias is shown in Figure \ref{fig:bias_example_weat}. It shows a clearly biased example where both occupations (secretary and engineer) would be considered biased due to our definition. However, since they achieve the same \weatw\ score, these cancel out in the effect size if put in contrary groups X,Y.
This issue arises, because WEAT separates the neutral words into groups according to their assumed stereotypes. This works well as a contrasting mechanism as long as the assumptions hold. If not, like in this example, biased words might not contribute to \weat's magnitude or if representing stereotypes counter-wise to the assumption such a pair would cancel out the biases of other pairs. If each word in $X$ had an equally biased counterpart in $Y$ one would report an effect size of $0$ over a set of arbitrarily biased words.\\
On the other hand, if indeed all words in $X$ and $Y$ had no bias and thus \weatw$(\mathbf{w}) = 0 \forall \mathbf{w} \in X \cup Y$, \weat\ is not defined due to its denominator being zero.


\textbf{$\mathbf{MAC}_{word}$ and $\mathbf{MAC}$ are not trustworthy:}
Consider the example from Figure \ref{fig:bias_example_angles} with $\theta = \pi$. Then the MAC score for secretary is:
\begin{align}
MAC_{word}(\mathbf{secretary}) &= \frac{1}{2} ((1-cos(\alpha)) + (1-cos(\pi-\alpha))) \\
&= 1.
\end{align}
For MAC, a score of 1 implies perfectly fair embeddings. In our case this score is reached independent of $\alpha$. However, considering the figure and our definition of bias, we clearly see that secretary would be biased for most choices of $\alpha$.\\
As a second example, if we considered $\alpha = \frac{\theta}{2}, \theta \neq \pi$, $\mathbf{secretary}$ would be represented equidistant to both gender attributes and thus considered neutral. However the MAC score would be 
\begin{align}
MAC_{word}(\mathbf{secretary}) &= \frac{1}{2} ((1 - cos(\alpha)) + (1 - cos(\theta - \alpha))) \\
&= 1 - cos\left(\frac{\theta}{2}\right),
\end{align}
i.e. it would always report a certain amount of bias, although the occupation's representation is perfectly fair. This issue extends to \mac, which is computed over a set of words $W$.


\textbf{$\mathbf{DirectBias}_{word}$ and $\mathbf{DirectBias}$ are not trustworthy:}
Consider Figure \ref{fig:bias_example_direction}. It shows a simplified example with two pairs of gender attributes, whereby the gender directions of the individual pairs differ significantly. Along the x-axis both gender directions (he-she, man-woman) agree, but they differ along the y-axis. Now, if we calculate a shared gender direction either by mean (which aligns with WEAT's intuition and our definition) or by the PCA approach described by Bolukbasi et al. \cite{bolukbasi} the results contradict each other. This has two reasons: Bolukbasi et al. compute the PCA over samples derived from multiple word pairs (e.g. he,she). For each word, they derive a sample like $\mathbf{he} - \mathbf{\mu}_{\mathbf{he},\mathbf{she}}$ and $\mathbf{she} - \mathbf{\mu}_{\mathbf{he},\mathbf{she}}$ with $\mathbf{\mu}_{\mathbf{he},\mathbf{she}}$ the mean of both vectors. The first principal component, which is used as the bias direction, aligns with the direction of maximum variance. One would expect that this is similar to the individual bias directions. However, the more these individual direction vary the more likely does the PCA bias direction differ from them. And in extreme cases as depicted in Figure \ref{fig:bias_example_direction}, it can be even contrary to the mean bias direction.\\
If we had a word aligning with the y-axis in the example, it would be considered neutral given the mean gender direction (and our definition), but maximally biased using the PCA bias direction. Hence, the Direct Bias is not trustworthy w.r.t. our definition.
